An evidence-based assumption that helps to reduce the discrepancy between the observed and predicted $^7$Be abundances in novae

Recent spectroscopic measurements of the equivalent widths of the resonant Be II doublet and Ca II K lines and their ratios in expanding nova ejecta indicate surprisingly high abundances of $^7$Be with a typical mass fraction $X_\mathrm{obs}(^7\mathrm{Be}) = 10^{-4}$. This is an order of magnitude larger than theoretically predicted values of $X_\mathrm{theor}(^7\mathrm{Be})\sim 10^{-5}$ for novae. We use an analytical solution of the $^7$Be production equations to demonstrate that $X_\mathrm{theor}(^7\mathrm{Be})$ is proportional to the $^4$He mass fraction $Y$ in the nova accreted envelope and then we perform computations of 1D hydrostatic evolution of the $1.15\,M_\odot$ CO nova model that confirm our conclusion based on the analytical solution. Our assumption of enhanced $^4$He abundances helps to reduce, although not completely eliminate, the discrepancy between $X_\mathrm{obs}(^7\mathrm{Be})$ and $X_\mathrm{theor}(^7\mathrm{Be})$. It is supported by UV, optical and IR spectroscopy data that reveal unusually high values of $Y$ in nova ejecta. We also show that a significantly increased abundance of $^3$He in nova accreted envelopes does not lead to higher values of $X_\mathrm{theor}(^7\mathrm{Be})$ because this assumption affects the evolution of nova models resulting in a decrease of both their peak temperatures and accreted masses and, as a consequence, in a reduced production of $^7$Be.

==> astronomy.tex <==
% astronmoy macro
% mostly objects
\newcommand{\ocen}{\mbox{$\Omega$ Cen}}


==> constants.tex <==
%constants
\newcommand{\kB}{\ensuremath{k_\mathrm{B}}} %Boltzmann's constant
\newcommand{\pF}{\ensuremath{p_\mathrm{F}}} %Fermi momentum
\newcommand{\EF}{\ensuremath{\mathcal{E}_\mathrm{F}}} %Fermi energy
\newcommand{\NA}{\ensuremath{N_\mathrm{\!A}}} %Avogadro number
\newcommand{\mb}{\ensuremath{m_\mathrm{u}}} %mean nucleon mas
\newcommand{\me}{\ensuremath{m_\mathrm{e}}} %electron mass
\newcommand{\mpr}{\ensuremath{m_\mathrm{p}}} %proton mass
\newcommand{\mn}{\ensuremath{m_\mathrm{n}}} %neutron mass
\newcommand{\alphaF}{\ensuremath{\alpha_\mathrm{F}}} %Fine structure


==> vectors.tex <==
%=======================================================================
%
% vectors.tex---some basic vector operators
%
% Requires package bm.sty
%
%=======================================================================

\RequirePackage{bm}
%\RequirePackage{amssymb}
%\RequirePackage{amsbsy}
\newcommand{\bvec}[1]{\ensuremath{\boldsymbol{#1}}} %boldface vector style
\newcommand{\grad}{\bvec{\nabla}} %gradient
\newcommand{\divr}{\nabla \cdot} %divergence
\newcommand{\curl}{\bvec{\nabla \times}} %curl
\newcommand{\lap}{\ensuremath{\nabla^2}} %Laplacian
\newcommand{\btens}[1]{\ensuremath{\boldsymbol{\mathsf{#1}}}}
\newcommand{\vcross}{\bvec{\times}}
\newcommand{\vdot}{\bvec{\cdot}}
% end vectors.tex

